Spatial Optimization of Interconnected Systems in Non-Convex Design Spaces

This paper presents a spatial optimization methodology that extends the Spatial Packaging of Interconnected Systems with Physical Interaction (SPI2) framework to support arbitrary, non-convex design boundaries. We introduce a smooth, differentiable inside-outside evaluation for components represented using the Maximal Disjoint Ball Decomposition (MDBD) method. The framework also incorporates center-of-gravity and moment-of-inertia calculations directly into the optimization, and provides an end-to-end computer-aided design (CAD) workflow for importing components and reconstructing the optimized assembly. The method is demonstrated on a fictional aircraft auxiliary unit. Results show that the optimizer can place multiple interconnected components within a custom geometry while simultaneously handling routing and physics-based objectives. The approach maintains geometric feasibility within numerical tolerance and illustrates the potential of MDBD-based SPI2 methods for practical engineering design applications.

==> Text/OptimizationFrameworks.tex <==
In this section, three optimization frameworks are presented to solve the placement and routing problem. As stated previously, the problems are constrained, non-linear, non-convex, and continuous; therefore, nonlinear programming (NLP) methods are used.

In this context, the interior-point optimization solver IPOPT from CasADi~\cite{CasADi, IPOPT} was adopted as the primary solver due to its robust constraint handling and Python integration. Unlike the Method of Moving Asymptotes (MMA) or ADAM, IPOPT provides Lagrange multiplier updates and second-order convergence properties, which are useful handeling a large number of constraints.

However, due to the highly non-linear nature of the placement and routing problem, the likelihood of convergence to a poor local optimum is high. To improve the chances of identifying better local optima, a \emph{nested hybrid} strategy is adopted. This combines stochastic exploration with deterministic gradient-based refinement via IPOPT. The problem is initialized multiple times, and the solver refines each initialization until convergence. By repeating this process until an exit condition is met, the framework increases the likelihood of finding the best local solution.

Given the exponential growth of computational complexity with system size, decomposition methods are also considered to enhance scalability. In particular the decomposition strategy Analytical Target Cascading (ATC)~\cite{ATC, ATC2, ATC3} are explored. ATC enables large, coupled problems to be partitioned into smaller subproblems that can be solved in parallel while maintaining system-level consistency.

Three frameworks are presented in total: a purely nested approach, a nested approach with ATC, and a nested approach combining the Geometric Projection Method (GPM) with MDBD, referred to as the \emph{Sphere of Influence} (SOI) approach. It must be noted that the full placement and routing problem is solved only with the first optimization framework, while the ATC and SOI approaches focus exclusively on the placement problem.

Before discussing these frameworks in detail, the methods used to initialize the interior-point solver are first described.
\subsection*{Initialization methods}
There are four initialization methods: Genetic Algorithm, Random Initialization, Equally Spaced, and manual initialization. 

The Genetic Algorithm used is from the PyMoo library \cite{Pymoo}. A Genetic Algorithm is an evolutionary optimization method inspired by natural selection. It begins with an initial population of candidate solutions, in our case, the design variables \(\mathbf{x}\), which is generated by random initialization. Each individual design variable is evaluated by the nested, ATC, or SOI algorithm. The survival step determines which individuals are retained, typically following the principle of \textit{“survival of the fittest.”} During selection, individuals are chosen as parents based on their fitness. The crossover operator then combines parents to produce offspring. Finally, mutation introduces small random variations in offspring with a certain probability, maintaining diversity and helping the algorithm avoid premature convergence \cite{Pymoo}.

Next, the Random Initialization function is similar to the first step of the genetic algorithm, as it provides a random selection of design variables \(\mathbf{x}\). The benefit of including both the random and genetic algorithms is that it can be determined whether the evolutionary aspect of the genetic algorithm yields better results than full random.

In addition, we also have an \textit{"equally spaced"} initialization scheme. This initialization places objects and routing nodes in "logical" starting positions by spacing them apart to the corners or halfway points in the design space. This still has a random component; however, it produces a more predictable initial position.

Finally, manual initialization allows a single initialization to be run from a user-specified location.

These initialization methods are used with the algorithms described further in this section.

\subsection*{Nested Framework}
\begin{figure}[t]
\centering
\includegraphics[width=8.9cm]{Figures/NestedApproach_Small.pdf}
\caption{Overview of the Nested Approach algorithm. Step A: creation of the MDBD objects. Step B: initialization of object positions and routings. Step C: selection of the initialization method. Step D: evaluation of the exit condition. Step E: optimization using CasADi’s IPOPT solver. Step F: output of the final object placements and routing results.}
\label{fig:Appendix:Nested Aproach}
\end{figure}

The nested framework, shown in Fig.~\ref{fig:Appendix:Nested Aproach}, uses one of four initialization methods to generate an initial position. This initial position, \(\mathbf{x}_0\), is used together with optimization problem~\ref{prob:1} or~\ref{prob:2}, which is solved using CasADi’s IPOPT algorithm~\cite{CasADi}. The resulting objective function value \(f(\mathbf{x}_\mathrm{opt})\) and corresponding design variables \(\mathbf{x}_\mathrm{opt}\) are then returned. These results are stored and used to generate a new initial design variable \(\mathbf{x}_0\)

in the next iteration. The process continues until the exit condition is met, such as reaching a specified number of random initializations or convergence of the genetic algorithm. Once this condition is satisfied, the best objective function value and its corresponding design variables \(\mathbf{x}_\mathrm{opt}\) are selected, from which the final object positions and routing configuration are determined.

\subsection*{Analytical Target Cascading}
Analytical Target Cascading (ATC) is an optimization method designed to solve hierarchical or multilevel optimization problems by decomposing them into smaller, interrelated subproblems~\cite{ATC}. The idea is that this hierarchical decomposition allows complex design problems to be solved more efficiently, supports parallelization, and often improves convergence properties compared to solving a single large-scale problem directly.

In this paper, an initial implementation of ATC is introduced for the placement problem. In this formulation, the routing aspect is omitted, and only the spatial placement of the MDBD objects is considered. As shown in Fig.~\ref{fig:ATC_Structure}, the framework is still very similar to the nested approach, in which a value is provided by an initialization that consists of a system-level component and multiple subsystems, each corresponding to an individual object.

\begin{figure}[t]
    \centering
    \includegraphics[width=8.9cm]{Figures/ATC.drawio.pdf}
    \caption{Overview of the Analytical Target Cascading (ATC) framwork. Step A: creation of the MDBD objects. Step B: initialization of object positions and routings. Step C: selection of the initialization method. Step D: evaluation of the exit condition. Step ATC: ATC using CasADi’s IPOPT to iteratively solve Problem \ref{prob:3}. Step F: output of the final object placements and routing results.}
    \label{fig:ATC_Structure}
\end{figure}

At the system level, the following optimization problem is defined:

\begin{prob}\label{prob:3}
System-Level Optimization Problem
\begin{equation*}
\begin{aligned}
& \min_{\mathbf{x}} && f_\mathrm{v}(\mathbf{x}) + \frac{1}{2}\sum^{n}_{i=1} \pi \|\mathbf{x}^u_i-\mathbf{x}^L_i\|^2 \\
& \text{s.t.} && \mathbf{g}^{\mathrm{obj\mbox{-}obj}}(\mathbf{x}) \leq 0,
\end{aligned}
\end{equation*}
\end{prob}

where \(f_\mathrm{v}\) represents the total volume of the placed objects, \(\mathbf{g}^{\mathrm{obj\mbox{-}obj}}\) are the object--object non-overlap constraints, and \(\pi\) is the scalar coupling parameter (or \emph{trust parameter}) that penalizes deviation between the system-level decisions \(\mathbf{x}^u_i\) (upper-level variables) and the subsystem responses \(\mathbf{x}^L_i\). The design variable \(\mathbf{x}\) is defined by \(\mathbf{x} = [\mathbf{x}^u_1,\dots,\mathbf{x}^u_n]\).

At the subsystem level, each object \(i\) receives its corresponding upper-level decision variables \(\mathbf{x}^u_i\) and solves a local optimization problem of the form:

\begin{prob}\label{prob:4}
Subsystem Optimization Problem
\begin{equation*}
\begin{aligned}
& \min_{\mathbf{x}^L_i} && 10^{-4}\|\mathbf{x}^L_i\|^2 + \boldsymbol{\lambda}_i^\mathrm{T}(\mathbf{x}^L_i - \boldsymbol{\gamma}_i) + \frac{1}{2}\rho\|\mathbf{x}^L_i - \boldsymbol{\gamma}_i\|^2 \\
& \text{s.t.} && \mathbf{g}^{\mathrm{obj\mbox{-}obj}}(\mathbf{x}^L_i,\,\mathbf{x}^u_i) \leq 0,
\end{aligned}
\end{equation*}
\end{prob}

where \(\boldsymbol{\gamma}_i\) denotes the target position communicated from the system level, \(\mathbf{x}^u_i\) are the shared or upper-level variables influencing subsystem \(i\), \(\boldsymbol{\lambda}_i\) is the dual variable enforcing consistency, and \(\rho\) is the penalty weight that determines how strongly each subsystem follows its assigned target.

The ATC process proceeds iteratively. In each outer iteration, the system broadcasts the updated targets \(\boldsymbol{\gamma}_i\) and upper-level variables \(\mathbf{x}^u_i\) to all subsystems. Each subsystem then solves its local problem and returns its response \(\mathbf{x}^L_i\). The system-level problem is subsequently solved as a \emph{repair step}, restoring feasibility by enforcing the non-overlap constraints and minimizing the total volume.

In less abstract terms, this means that the system minimizes the total volume comprised by the components by setting targets to each of the subsystems. In the subsystem, one MDBD object is moved while all other objects are fixed. By enforcing the constraints, updating the targets, and gradually increasing the coupling and penalty parameters, the system converges to a point where an optimum is reached and \(\mathbf{x} = \mathbf{x}^u = \mathbf{x}^L\). A more detailed explanation on the the targets are updated can be found in Appendix~\ref{Appendix:C}.

\subsection*{Sphere of Influence}
\begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/SOI.pdf}
    \caption{Object Spheres \(b_{i,\mu}\) (1, Light Purple), and Encompassing Sphere (Sphere of Influence) (2, red). Where an overlap in the Encompassing Spheres is seen}
    \label{fig:Appendix:SOI}
\end{figure}

The final placement approach combines the Geometric Projection (GPM) and Maximal Disjoint Ball Decomposition (MDBD) method to reduce the number of constraint equations. Each object’s MDBD representation is enclosed by a larger GPM sphere. When two GPM spheres are non-overlapping, their corresponding MDBD objects are certainly non-interfering, and no detailed checks are required. However, if two GPM spheres touch or intersect, the objects enter a Sphere of Influence (SOI), where detailed MDBD-level distance constraints are activated, as can be seen in Fig.~\ref{fig:Appendix:SOI}. When the enclosing spheres are disengaged, there are, in this case, two object-object constraint equations. When the enclosing spheres are engaged, there are 25 object-object constraint equations active.

\begin{figure}[t]
    \centering
    \includegraphics[width=8.9cm]{Figures/DiagramSOI.drawio.pdf}
    \caption{Overview of the Sphere of Influence algorithm. Step A: creation of the MDBD objects, including enclosing sphere. Step B: initialization of object positions. Step C: selection of the initialization method. Step D: evaluation of the exit condition. Step E1: check which constrains must be active based on enclosing spheres, Step E2: optimization using CasADi’s IPOPT solver. Step F: output of the final object placements and routing results.}
    \label{fig:Appendix:SOIDiagram}
\end{figure}

In implementation, an active-set strategy switches the number of constraints during optimization. Initially, only the enclosing-sphere constraints are used for all object pairs, thereby minimizing the problem size. When GPM spheres overlap, those object pairs are marked active, and the optimizer adds all corresponding MDBD object-object constraints for that subset. After each solve, true sphere-to-sphere clearances are evaluated; if interference persists, the constraint set expands until all pairs are feasible. This adaptive constraint activation maintains a minimal set of constraints while maintaining collision-free placement.

==> Text/Placement_Optimization.tex <==
The placement of components is an NP-Hard problems where with more parts, and in this case, more spheres, the number of computations increases with
\begin{equation}
    n_{\mathrm{c}} = \frac{n_{\mathrm{o}}(n_{\mathrm{o}}-1)}{2}n_{\mathrm{s}}^2
\end{equation},
where $n_{\mathrm{eq}}$ is the number of equations, $n_{\mathrm{o}}$ the number of objects, and  $n_{\mathrm{s}}$ the number of spheres per object. Naturally, this assumes that all objects have an equal number of spheres, which might not be the case in use, however, is the worst case scenario.

\subsection{Objective Function}
The aim is to configure all the parts of a system as compact as possible, but what does compact design mean? In short, compactness generally refers to the degree to which an object or system occupies a minimal amount of space. However, in engineering reality, compactness can also refer to the possibility of a system to fit within the restricted volume of another system. To define this mathematically, this author takes three different definitions; Bounded Box Volume, minimal object to object distance, and minimal volume between the parts. Due to the nature of MDBD, being an approximation of the actual object, the latter definition might not be suitable. Thus two definitions remain, which can be used to create an objective function.

\begin{equation}
f_\mathrm{v}(\textbf{x}) = \prod_{k=1}^{k=n} \left(
\max_{\forall \mathrm{b}_{i} \in \mathcal{B}} \left( \textbf{p}_{\mathrm{b}_i}^{(k)} + r_{\mathrm{b}_i} \right)
-
\min_{\forall \mathrm{b}_i \in \mathcal{B}} \left( \textbf{p}_{\mathrm{b}_i}^{(k)} - r_{\mathrm{b}_i} \right)
\right)
\end{equation}

Where $f_v(x)$ is the total volume of the bounding box, which can be used as the objective function, $n$ is the number of dimensions, the set of spheres in all MDBD models is denoted as $\mathcal{B}$, the centre position of each sphere as $\textbf{p}_{\mathrm{b}_i}$, and the radius $r_{\mathrm{b}_i}$. $\mathcal{P}$


And for differential purposes a min or max operator cannot be used as these are not differentiable. Thus a custom operator will be used, which will create differentiability.

The Boltzmann operator is used to create a smooth minimum and a smooth maximum for the volume objective function, substituting the minimum and maximum operator, the goal of this is to create a function which is continuous and differentiable.  

Given a vector of values \( \mathbf{v} = [v_1, v_2, \dots, v_n] \), the function approximates the maximum value of \( \mathbf{v} \) using a weighted average with exponential weights:

\[
f_\mathrm{smooth}(\mathbf{v}, \alpha) = \frac{\sum_{i=1}^{n} v_i \, e^{\alpha v_i}}{\sum_{i=1}^{n} e^{\alpha v_i}}
\]

Where:
\begin{itemize}
    \item \( \alpha > 0 \) controls the sharpness of the approximation (higher \( \alpha \) makes the result closer to \( \max(\mathbf{v}) \))
    \item The function is smooth and differentiable, making it suitable for gradient-based optimization
\end{itemize}


And for the mean distance approach


Assume:
\begin{itemize}
    \item There are $K$ objects: $O_1, O_2, \dots, O_K$.
    \item Each object $O_k$ contains $M_k$ points: $\{P_j^{(k)}\}_{j=1}^{M_k}$.
\end{itemize}

We define the mean pairwise distance between all points from different objects as:

\begin{equation}
f(\{O_k\}_{k=1}^K) = \frac{1}{S} \sum_{1 \leq a < b \leq K} \sum_{i=1}^{M_a} \sum_{j=1}^{M_b} \left\| P_i^{(a)} - P_j^{(b)} \right\|
\end{equation}

where
\begin{equation}
S = \sum_{1 \leq a < b \leq K} M_a \cdot M_b
\end{equation}

Here:
\begin{itemize}
    \item The outermost sum iterates over all unique unordered pairs of objects $(a, b)$.
    \item The inner sums iterate over all pairs of points from object $O_a$ and $O_b$.
    \item $S$ is the total number of inter-object point pairs.
\end{itemize}






%def smooth_min(a, b, alpha=10):
%    return -(1/alpha) * log(exp(-alpha * a) + exp(-alpha * b))

\subsection{Constraint Function}



==> Text/TheDiscussion.tex <==
A few comments are in order, the results are all run once, which makes the results for the initialization 

especially for the initialization 

==> Text/TheUseCase.tex <==
%To test the algorithm effectively, we need to be able to evaluate input and output. As stated before, the problem is non-linear and non-convex, thus a global optimal solution cannot be guaranteed. Therefore, we need to construct a use-case is such a way that a person can judge if the results produced by the algorithm make sense.

\subsection{Benchmark Comparison with Prior Work}
A use case defined in a previous study at the University of Connecticut~\cite{Behzadi} is adopted to enable a direct and fair comparison. This allows an objective evaluation between the stochastic gradient descent (SGD) approach of~\cite{Behzadi} and the nested optimization framework developed in this work.

In the original use case, configurations of three, four, and six cubes (each measuring 1.5 × 1.5 × 1.5) were analyzed, each containing 100 MDBD spheres. The cubes were connected by three routing segments that start and end at the center of each MDBD object. The reported quantities include the total volume of the axis-aligned bounding box and the total routing length.

The most relevant setup parameters are summarized in Table~\ref{tab:Apples}. The Genetic Algorithm (GA) is used for initialization. Configurations with 3, 4, and 6 objects are evaluated across various use cases, with three routing segments (two control points) in each. Problem~\ref{prob:1} is solved using the objective functions \(f_1(\mathbf{x})\) and \(f_2(\mathbf{x})\) The objects are modeled as cubes filled with 14, 25, 50, or 100 MDBD spheres, and the optimization algorithm applied is the nested approach. The comparison with exponential routing, denoted by \(f_2(\mathbf{x})\) in Table~\ref{tab:Apples}, is performed only for configurations with 25 spheres per object.

In total, fifteen use cases are evaluated, of which three (those with 100 spheres per object) can be directly compared to~\cite{Behzadi}. Testing multiple MDBD “resolutions” allows assessment of how solution quality varies with the number of spheres per object. Additional setup details are provided in Appendix~\ref{Appendix:E}, and corresponding results are discussed in Section~\ref{section:results}.
\begin{table}[t]
\centering
\small
\caption{Overview of the setup used for the benchmark comparison}
\label{tab:Apples}
\begin{tabularx}{\columnwidth}{l|X|X|X|X}
Parameter &  & &  & \\
\hline
Initialization & \centering Random & \centering -- & \centering -- & \centering -- \tabularnewline
Nr Objects & \centering 3 & \centering 4 & \centering 6 & \centering -- \tabularnewline
Nr Spheres & \centering 14 & \centering 25 & \centering 50 & \centering 100 \tabularnewline
Nr Control Points & \centering 2 & \centering -- & \centering -- & \centering -- \tabularnewline
Problem & \centering 1 & \centering -- & \centering -- & \centering -- \tabularnewline
Objective Function & \centering \(f_1(\mathbf{x})\) & \centering \(f_2(\mathbf{x})\) & \centering -- & \centering -- \tabularnewline
Objects & \centering Cubes & \centering -- & \centering -- & \centering -- \tabularnewline
Algorithm & \centering Nested & \centering -- & \centering -- & \centering -- \tabularnewline
\end{tabularx}
\end{table}

\subsection{Novel Benchmark Use-Cases}
As stated previously, the placement and routing problem is a constrained, non-linear, non-convex, and continuous optimization problem. By definition, global optimality cannot be guaranteed or verified. Therefore, a use case is needed where it can be analytically determined whether the desired result is achieved. As shown in the results, this is not possible for the use case introduced in \cite{Behzadi}.  

To address this limitation, several new benchmark cases are introduced to evaluate the performance and robustness of the optimization algorithms. One of the main challenges in this problem is navigating the non-linear loss field. When symmetric use cases are introduced, multiple distinct configurations can yield identical objective values. For example, when placing two identical cubes, there are 144 configurations that lead to the same minimal volume, indicating a high degree of symmetry.  

For routing, the resulting configuration must also be logically interpretable and analytically optimal. Additionally, the objectives should not be conflicting: when the volume is minimal, the routing distance should be minimal as well. This is particularly important since IPOPT from CasADi does not directly handle multi-objective optimization.

Based on these considerations, three novel benchmark use cases are defined: one with high symmetry, one with reduced symmetry, and one with a unique configuration.

\subsubsection{Cuboids}
\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/Cuboid.pdf}
    \caption{Cuboid Schematic: the dimensions 1x1x2 are shown in the single cuboid on the left; the port of the cuboid is shown in green. Note that there are two ports; only the bottom one is not visible. On the right-hand side of the figure, an analytical optimal configuration of 6 cuboids with routing is shown.}
    \label{fig:Cuboid}
\end{figure}
For the high-level of symmetry case, a rectangular 1x1x2 shape is used with two ports for routing. These ports are connected at the long end. Fig.~\ref{fig:Cuboid} displays the geometry of one object on the left-hand side and 6 objects on the right-hand side. The port connectivity for two objects is as follows \(\mathrm{connections} = [(\varphi_{1,1},\varphi_{2,1}), (\varphi_{1,2},\varphi_{2,2})]\) which means that port one of object one is connected to port one of object two, and port two of object one is connected to port two of object two. This scales for four and six objects, as shown in Fig.\ref{fig:Cuboid}. This use case provides multiple analytical optimal configurations. For two objects, the volume should be four and the routing length two, for four objects eight and four, and for six objects twelve and six. Additionally, the optimal positions should be easily distinguishable from non-optimal ones.

In terms of symmetry, for two objects, there are sixteen possible configurations that are equally minimal in both volume and routing. For four objects, 44 configurations, and with six objects, 136 configurations.

\subsubsection{L-shapes}
\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/L_Shape.pdf}
    \caption{L-Shape Schematic; with on the left a single L-shape and on the right an analytical optimum of six L-shaped objects is displayed.}
    \label{fig:L_Shape}
\end{figure}
To reduce the number of possible configurations, we can also use an L-shape with routing, as shown in Fig.~\ref{fig:L_Shape}. The port connectivity for two objects would be \(\mathrm{connections} = [(\varphi_{1,1},\varphi_{2,2}), (\varphi_{1,2},\varphi_{2,1})]\).

The use case provides an analytical optimum: for two objects, the minimal volume is six with a minimal routing distance of two; for four objects, the minimal volume is twelve with a routing distance of four; and for six objects, the minimal volume is eighteen with a routing distance of six. An example of the configuration is shown on the right-hand side of Fig.~\ref{fig:L_Shape}. 

For two L-shaped objects, the configuration is unique. For four objects, there are eight possible configurations, and for six objects, there are 48 configurations.

\subsubsection{Unique}
\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/Unique.pdf}
    \caption{Unique benchmark schematic. The left shows the double L-shape geometry. On the right, this double L-shape is combined with two L-shapes and one cuboid, forming a configuration with five routing paths. The L-shapes are also connected to the double L-shape at the bottom.}
    \label{fig:Unique}
\end{figure}
The final benchmark represents a unique configuration, meaning that only one solution exists. As discussed in the previous section, the two-object L-shape already yields a unique arrangement. Here, the objective is to construct a similarly unique use case for four objects to enable direct comparison with the symmetric cuboid and L-shape benchmarks. A six-object version is omitted, as the focus is on examining how symmetry influences the number of analytical optima identified by the initialization algorithms.

As shown in Fig.~\ref{fig:Unique}, the configuration consists of a new base geometry on the left, combined with two L-shapes and one cuboid featuring distinct port positions. The total volume of the configuration is twelve, and the routing length is five, with two routing connections located on the underside (not visible in Fig.~\ref{fig:Unique}). The corresponding MDBD representations of these objects are provided in Appendix~\ref{Appendix:F}.

\subsection{Test Plan: What to Test and Why}
The aim of this study is to evaluate whether the proposed nested hybrid framework can solve spatial placement and routing \emph{accurately} and \emph{efficiently}, and to understand when alternative formulations (constraints, decomposition, routing objectives) help or hurt. Following the gaps identified in the introduction, we structure the tests around six questions:

\begin{itemize}
    \item Accuracy vs.\ ground truth (Cuboid benchmark): How close are converged solutions to analytical optima?
    \item Robustness to initialization: How sensitive are outcomes to Equally Spaced (ES), Genetic Algorithm (GA), and Random starts?
    \item Symmetry: How does problem symmetry (Cuboid, L-shape, Unique) affect the share of near-optimal solutions?
    \item Framework choice: How do Nested, ATC, and SOI compare in objective value and runtime on identical tasks?
    \item Constraint and objective formulations: What is the trade-off between Absolute vs.\ Soft-Sum constraints, and between quadratic vs.\ exponential routing objectives?
    \item Scalability and resolution: How do iteration-level times scale with numbers of objects, spheres (MDBD resolution), and routing control points; and does warm-starting from lower resolution help?
\end{itemize}

Across tests, solver tolerances, penalty weights, bounds, and stopping criteria are held fixed. When comparing frameworks (Nested/ATC/SOI) or formulations (Absolute/Soft-Sum; quadratic/exponential routing), only the factor under study is varied.

Table~\ref{tab:TestInit} lists the experimental factors and levels used throughout the study. Not all combinations are exercised; we select minimal, targeted subsets per research question (full schedule in Appendix~\ref{Appendix:G}).
\begin{table}[t]
\centering
\small
\caption{Experimental factors and levels used across tests}
\label{tab:TestInit}
\begin{tabularx}{\columnwidth}{l|X|X|X}
Parameter & Setting A & Setting B & Setting C \\
\hline
Initialization & \centering Random & \centering GA & \centering ES \tabularnewline
Nr Objects & \centering 2 & \centering 4 & \centering 6 \tabularnewline
Nr Spheres & \centering 20 & \centering 40 & \centering 60 \tabularnewline
Nr Control Points & \centering no routing & \centering 2 & \centering 4 \tabularnewline
Problem & \centering 1 & \centering 2 & \centering -- \tabularnewline
Objective Function & \centering \(f_3(\mathbf{x})\) & \centering \(f_4(\mathbf{x})\) & \centering -- \tabularnewline
Objects & \centering Cuboids & \centering L-shape & \centering Unique \tabularnewline
Algorithm & \centering Nested & \centering ATC & \centering SOI \tabularnewline
\end{tabularx}
\end{table}
\begin{table}[t]
\centering
\small
\caption{Warm-start schedule from 20-sphere solutions (Cuboid).}
\label{tab:ByHand}
\begin{tabularx}{\columnwidth}{l|X|X|X}
Parameter & Setting A & Setting B & Setting C\\
\hline
Initial Position & \centering best \(\mathbf{x}_0\) & \centering \(\mathbf{x}_\mathrm{opt}\) & \centering -- \tabularnewline
Nr Objects & \centering 2 & \centering 4 & \centering 6 \tabularnewline
Nr Spheres & \centering 30 & \centering 40 & \centering -- \tabularnewline
Nr Control Points & \centering no routing & \centering 2 & \centering -- \tabularnewline
Problem & \centering 1 & \centering -- & \centering -- \tabularnewline
Objective Function & \centering \(f_3(\mathbf{x})\) & \centering -- & \centering -- \tabularnewline
Objects & \centering Cuboids & \centering -- & \centering -- \tabularnewline
Algorithm & \centering Nested & \centering -- & \centering -- \tabularnewline
\end{tabularx}
\end{table}
%\begin{table}[t]
%\centering
%\small
%\caption{Experimental factors and levels used across tests (subsetted per question).}
%\label{tab:TestInit}
%\begin{tabularx}{\columnwidth}{@{}l *{3}{>{\centering\arraybackslash}X}@{}}
%\toprule
%\textbf{Factor} & \textbf{Level A} & \textbf{Level B} & \textbf{Level C} \\
%\midrule
%Initialization & Random & GA & ES \\
%Objects (count) & 2 & 4 & 6 \\
%MDBD spheres / object & 20 & 40 & 60 \\
%Routing control points & none & 2 & 4 \\
%Constraint formulation & Absolute (Prob.~\ref{prob:1}) & Soft-Sum (Prob.~\ref{prob:2}) & -- \\
%Routing objective & $f_3(\mathbf{x})$ (quadratic) & $f_4(\mathbf{x})$ (exponential) & -- \\
%Geometry class & Cuboid & L-shape & Unique \\
%Framework & Nested & ATC & SOI \\
%\bottomrule
%\end{tabularx}
%\end{table}

To study resolution scaling, we warm-start higher-resolution runs from a previously best solution at lower resolution. Two seeds are used: the best found initial point $\mathbf{x}_0$ and the best converged solution $\mathbf{x}_{\mathrm{opt}}$ at 20 spheres. Higher-resolution targets use 30–40 spheres with and without routing (Table~\ref{tab:ByHand}).

%\begin{table}[t]
%\centering
%\small
%\caption{Warm-start schedule from 20-sphere solutions (Cuboid).}
%\label{tab:ByHand}
%\begin{tabularx}{\columnwidth}{@{}l *{3}{>{\centering\arraybackslash}X}@{}}
%\toprule
%\textbf{Parameter} & \textbf{Setting A} & \textbf{Setting B} & \textbf{Setting C} \\
%\midrule
%Warm-start seed & best $\mathbf{x}_0$ & $\mathbf{x}_{\mathrm{opt}}$ & -- \\
%Objects (count) & 2 & 4 & 6 \\
%Target spheres / object & 30 & 40 & -- \\
%Routing control points & none & 2 & -- \\
%Constraint formulation & Absolute (Prob.~\ref{prob:1}) & -- & -- \\
%Routing objective & $f_3(\mathbf{x})$ (quadratic) & -- & -- \\
%Geometry class & Cuboid & -- & -- \\
%Framework & Nested & -- & -- \\
%\bottomrule
%\end{tabularx}
%\end{table}

Exercising Table~\ref{tab:TestInit} combinatorial would yield 2{,}916 cases and is out of scope. We therefore test only the contrasts needed to answer the six questions above, matching the comparisons shown in the Results.

%\subsection{What to test and why}
%\begin{table}[t]
%\centering
%\small
%\caption{Overview of benchmark test parameters}
%\label{tab:TestInit}
%\begin{tabularx}{\columnwidth}{l|X|X|X}
%Parameter &  &  & \\
%\hline
%Initialization & \centering Random & \centering GA & \centering ES \tabularnewline
%Nr Objects & \centering 2 & \centering 4 & \centering 6 \tabularnewline
%Nr Spheres & \centering 20 & \centering 40 & \centering 60 \tabularnewline
%Nr Control Points & \centering no routing & \centering 2 & \centering 4 \tabularnewline
%Problem & \centering 1 & \centering 2 & \centering -- \tabularnewline
%Objective Function & \centering \(f_3(\mathbf{x})\) & \centering \(f_4(\mathbf{x})\) & \centering -- \tabularnewline
%Objects & \centering Cuboids & \centering L-shape & \centering Unique \tabularnewline
%Algorithm & \centering Nested & \centering ATC & \centering SOI \tabularnewline
%\end{tabularx}
%\end{table}
%
%
%In addition to test the difference with MDBD resolution
%
%\begin{table}[t]
%\centering
%\small
%\caption{Initialization by hand from previously best determined position using 20 spheres per object}
%\label{tab:ByHand}
%\begin{tabularx}{\columnwidth}{l|X|X|X}
%Parameter & & &  \\
%\hline
%Initial Position & \centering best \(\mathbf{x}_0\) & \centering \(\mathbf{x}_\mathrm{opt}\) & \centering -- \tabularnewline
%Nr Objects & \centering 2 & \centering 4 & \centering 6 \tabularnewline
%Nr Spheres & \centering 30 & \centering 40 & \centering -- \tabularnewline
%Nr Control Points & \centering no routing & \centering 2 & \centering -- \tabularnewline
%Problem & \centering 1 & \centering -- & \centering -- \tabularnewline
%Objective Function & \centering \(f_3(\mathbf{x})\) & \centering -- & \centering -- \tabularnewline
%Objects & \centering Cuboids & \centering -- & \centering -- \tabularnewline
%Algorithm & \centering Nested & \centering -- & \centering -- \tabularnewline
%\end{tabularx}
%\end{table}
%
%Now, we can use the geometries presented to create tests to evaluate the optimization frameworks presented in Section~\ref{section:Methods}. To revert back to the aim of this paper; we want to develop an optimization method to be able to solve the placement and routing problem accurately and efficiently.
%
%The nested approaches which all three algorithms have, highlight the two important sections of the problem. The initialization in the loss-field, and finding the local minima based on that initial position. One test is varying the initialization strategy and evaluating the results based on that.
%
%In addition, as presented in this section, it can also be checked how many logical optimal results are found based on the different symmetries. This can tell us something about the likeliness of finding a solution.
%
%There is also the problem of scalability of the constraints, which as will be seen in the results will have a considerable effect on solving time. There are multiple solution directions to attempt to reduce solving time and maintain solution accuracy. The first one is that instead of using absolute constraints to compare all spheres with all spheres, we use a soft-sum constraint as used in Problem.~\ref{prob:2}, the second is dividing the design space, which is what the ATC and SOI algorithm are trying to achieve, the third solution direction is the resolution of the amount of spheres and number of routing. Within this there are also two directions 
%
%
%To sum up, we test the comparison of; the initialization, the symmetry, the optimization framework, the constraint equation approach, the routing objective function, and the scalability based on the MDBD resolution. All the varied parameters can be seen in Table~\ref{tab:TestInit} and Table~\ref{tab:ByHand}. Naturally, with the items we want to test, not the entire Table~\ref{tab:TestInit} is tested in a combinatorial fashion, as this would result in 2916 test-cases, with on average 1 hour per test-case would simply take too long for this study. Thus only the direct comparisons for the stated curiosities will be tested. The complete test schedule can be found in Appendix~\ref{Appendix:G}.
